HElium: A Language and Compiler for Fully Homomorphic Encryption with Support for Proxy Re-Encryption

Privacy-preserving analysis of confidential data can increase the value of such data and even improve peoples' lives. Fully homomorphic encryption (FHE) can enable privacy-preserving analysis. However, FHE adds a large amount of computational overhead and its efficient use requires a high level of expertise. Compilers can automate certain aspects such as parameterization and circuit optimizations. This in turn makes FHE accessible to non-cryptographers. Yet, multi-party scenarios remain complicated and exclude many promising use cases such as analyses of large amounts of health records for medical research. Proxy re-encryption (PRE), a technique that allows the conversion of data from multiple sources to a joint encryption key, can enable FHE for multi-party scenarios. Today, there are no optimizing compilers for FHE with PRE capabilities. We propose HElium, the first optimizing FHE compiler with native support for proxy re-encryption. HElium features HEDSL, a domain-specific language (DSL) specifically designed for multi-party scenarios. By tracking encryption keys and transforming the computation circuit during compilation, HElium minimizes the number of expensive PRE operations. We evaluate the effectiveness of HElium's optimizations based on the real-world use case of the tumor recurrence rate, a well-known subject of medical research. Our empirical evaluation shows that HElium substantially reduces the overhead introduced through complex PRE operations, an effect that increases for larger amounts of input data.

==> dsl.tex <==
\section{HElium Language}
This section gives an overview of the domain-specific language of HElium and presents its features. 
HElium provides a domain-specific language (DSL) that abstracts FHE programs.
Scheme-specific details are hidden to improve the usability for less-experienced developers.
In this section, we will describe the language, and its features.
\begin{figure}
\caption{HElium Program: A mind-blowing title}
\begin{lstlisting}[language=HElium]
input a1: int @Key1 <= Party1;
input b1: int @Key1 <= Party1;
input a2: int @Key2 <= Party2;
input b2: int @Key2 <= Party2;
input a3: int @Key3 <= Party3;
input b3: int @Key3 <= Party3;

output sum: a1*b1 + a2*b2 + a3*b3;
output quantity: b1 + b2 + b3;
\end{lstlisting}
\label{lst:dsl-example}
\end{figure}

\subsection{Data Types}
HElium supports two base types: integer, fixed-point numbers.
On top of them it provides basic support for fixed-size arrays.
Depending on the targeted encryption scheme, the size of the inputs can have a significant impact on the execution runtime of FHE programs.
Consequently, it is beneficial to enable the developer to define the size of inputs granularly.
HElium allows to define an upper boundary for all inputs.
In some scenarios it can be necessary to differentiate between inputs.
Therefore, the base types of HElium are configurable, i.e., their size can be adjusted to the developers needs.
For example, a Boolean type can be represented through an integer of length $1$, i.e., \lstinline{int<1>}. 
This size parameter is optional.
HElium is designed as an abstraction layer on top of multiple HE schemes.
For backends that operate on Boolean circuits, the input sizes relates directly to the bit-length of inputs. 
In contrast, in backend with an integer encoding, the input size is translated to a corresponding plaintext modulus.
Techniques like batching can impose additional requirements on the plaintext modulus.
Therefore, the implementation of the data types can vary. 
%\ms{Something to arrays}
The type system further differentiates between encrypted and plaintext data.
Each variable is defined as encrypted per default, if it is not annotated with the qualifier \textit{plain}.
Encrypted represent ciphertext inputs and \textit{plain}-marked inputs plaintext values.
This behavior ensures security by default.

\subsection{Inputs and Outputs}
The compiler and its language can represent a multi-party scenario. 
Therefore, HElium programs may have multiple inputs and outputs, provided or targeting different parties.
It is possible to derive inputs and outputs of the program automatically, but it limits later optimization opportunities.
For example, for dead-code elimination, the compiler needs to know which parts of the program can be safely removed and which must be preserved. 
Therefore, in HElium, inputs and outputs of the program are specified explicitly and are named.
For each input or output it can be specified, the data-providing or data-using party, respectively.
Furthermore, a key label that represents an encryption key can be applied to inputs and outputs of the program.
Both, the participant and the key label are optional.
If they are omitted, the compiler suggests default values.
In lines ... to ... of Figure ..., the definition of inputs is depicted. 
Similarly to inputs, outputs are named. 
Outputs can be defined by \lstinline{output <name>: <expression>} as shown in lines ....
\ms{Add some references to the example program}
The inputs and outputs build the interface of the program.

\subsection{Operations}
The DSL of HElium provides different types of operations: arithmetic operations, vector-specific operations, Boolean operations, and comparison operations.
These operations are expressed by symbols. 
%\ls{ROT is currently not supported at least by BFV backend}

\begin{table}[t]
    \caption{Builtin Operations of HElium\ms{Ist so eine tabelle sinnvoll? }}
\label{tab:builtin-operations}
    \begin{tabular}{@{}llc@{}}
        \toprule
     \textbf{Symbol}                       & \textbf{Operation}      & \textbf{Argument / Result Type}\\
    \midrule
    +                            & Addition       & \multirow{4}{*}{\begin{tabular}[x]{@{}c@{}}(int | vector\textless{}int\textgreater{},int | vector\textless{}int\textgreater{}) \\$\rightarrow$ (int, vector\textless{}int\textgreater{})\end{tabular}} \\
    -                            & Substraction   &                                                                                                                                             \\
    *                            & Multiplication &                                                                                                                                             \\
    **                           & Power          &                                                                                                                                             \\
    \midrule
    \textgreater{}\textgreater{} & Right-Rotation & \multirow{2}{*}{\begin{tabular}[x]{@{}c@{}}(vector\textless{}int\textgreater{},int) \\$\rightarrow$ (vector\textless{}int\textgreater{})\end{tabular}} \\
     \textless{}\textless{}       & Left Rotation  &                                                                                                                                             \\
    \bottomrule
    \end{tabular}
\end{table}
Operations on vector data types are performed element-wise.
Scalar operands are treated as single-element vectors.
HElium is build with extensibility in mind. Therefore, it supports Boolean operations and comparisons.
However, these are out of scope of our current work.

\subsection{Function Definition}
To enable encapsulation of reusable code, HElium allows the definition of functions.
Functions are defined using the \textit{func} keyword followed by a function name and the argument signature.
Each function must contain a \textit{return} statement that marks the result of the function.
Since HElium is scoped, the body of a function has its own scope.
Therefore, variable definitions in the body of that function are only accessible within the function.
Functions can be invoked by their function name followed by their arguments.
The type parameters of the function arguments are optional.
HElium tries to determine the omitted type signature according to the provided arguments at the invocation.
If no types are assigned to the function signature, the behavior of the function depends on the types of the provided arguments.
Figure~\ref{lst:dsl-function-definition} depicts the definition of a function \textit{add} in HElium.
\begin{figure}
    \caption{Function Definition and Invocation}
\begin{lstlisting}[language=HElium]
func add(a,b) {
    return a + b;
}
var c = add(1, 2); // Calls the function
\end{lstlisting}
\label{lst:dsl-function-definition}
\end{figure}
\ms{@Mirko: check whether the compiler needs type information of the arguments...should not}
A function can take multiple arguments and has to return a value.
In addition to self-defined functions, HELium provides intrinsics, i.e, built-in functions.
For example, the function \lstinline{size()} returns the size of a vector.
Since the size of vectors is fixed and known at compile time, HElium can translate \textit{size($\cdot$)} directly to a numerical literal of the vector's size.
%\ls{Are there more intrinsics? I think this topic belongs to functions and not to operations.}
%\ls{There are two ways to to represent built-ins. One is by using intrinsics, i.e., having a transformation inside the compiler that replaces an op with a more efficient one. Or having a standard library written in the very language, e.g., as EVA's EXL.}

% \subsection{Branching on Encrypted Data}

% Due to the properties of HE, control-flow decisions on encrypted conditions cannot be made directly without access to the corresponding decryption key.
% \ls{Is the possibility to observe branches problematic?}
% However, there are mechanisms to emulate branching with HE. 
% One approach is the independent execution of branches. \ls{Is this overall possible with HE or only in specific schemes?}
% Followed by combination of the changes \ls{What means "combination of the changes?}, which are made in the branches, with \textit{MUX} operations.
% This approach typically adds additional computational overhead to the program.
% \ls{How does a result look like? How can a client program extract the correct result?}

% Listing~\ref{lst:dsl-if-then-else} depicts an example program including an \textit{if-then-else} structure.
% Based on the condition $a>b$, the program either returns $a$ or $b$, i.e., it returns the maximum $c=max(a,b)$. \ls{How can $a>b$ be homomorphically evaluated?}
% \begin{lstlisting}[language=HElium,label=lst:dsl-if-then-else,caption={If-Then-Else Branching Structure}]
% input a: int<20> <= Party1;
% input b: int<20> <= Party2;
% if (a>b) then {
%     output c = a;
% } else {
%     output c = b;
% }
% \end{lstlisting}

% The presented example shows an \textit{if-then-else} structure that operates as a conditional assignment.
% Based on the condition, either $a$ or $b$ is assigned to the output $c$.
% The DSL provides a short form of such conditional assignments: the ternary operator \begin{equation*}
%     \text{<condition>}?\text{<true-branch>}:\text{<false-branch>}.
% \end{equation*}
% Listing~\ref{lst:dsl-if-then-else-short} depicts the equivalent short form of the program shown in Listing~\ref{lst:dsl-if-then-else}.
% The given program represents the same function but with less program code.
% \begin{lstlisting}[language=HElium,label=lst:dsl-if-then-else-short,caption={Ternary Operator}]
% input a: int<20> <= Party1;
% input b: int<20> <= Party2;
% output c = (a>b) ? a : b;
% \end{lstlisting}
\subsection{Loops}
Next to functions, loops can help to improve readability and can enable code reuse.
Therefore, HElium implements \textit{for}-loops.
Loops in HElium have a behavior similar to \textit{for-each}-loop in other programming languages.
They provide a convenient way to iterate through the elements of a vector.
Listing~\ref{lst:dsl-for-loop} depicts a DSL program with a \textit{for}-loop.
The program calculates the sum of a vector $a$.
As shown in line $3$, a for-loop is constructed by the keyword $for$ followed by arguments and a block of statements in line $4$.
The first two arguments define new variables that give access to the current item and the current index, respectively.
Both are only accessible within the statement block.
The argument \textit{index} is optional.
The third argument requires a vector over which elements the for loops iterates.
\begin{figure}
    \caption{For-Loop in HElium}
\begin{lstlisting}[language=HElium]
input a: int[1024];
var sum: int = 0;
for (item, index : a) {
    sum = sum + item
}
\end{lstlisting}
\label{lst:dsl-for-loop}
\end{figure}
Homomorphic-encryption programs are subject to several branching and parameterization constraints.
As a result, branching or loops on ciphertext conditions can be computational expensive.
Therefore, HElium focuses on loops that have a boundary which can be determined at runtime.
This enables HElium to unroll loops during compilation and limits the additional computational complexity of loops.
